Cosmological lensing ratios with DES Y1, SPT and Planck

Correlations between tracers of the matter density field and gravitational lensing are sensitive to the evolution of the matter power spectrum and the expansion rate across cosmic time. Appropriately defined ratios of such correlation functions, on the other hand, depend only on the angular diameter distances to the tracer objects and to the gravitational lensing source planes. Because of their simple cosmological dependence, such ratios can exploit available signal-to-noise down to small angular scales, even where directly modeling the correlation functions is difficult. We present a measurement of lensing ratios using galaxy position and lensing data from the Dark Energy Survey, and CMB lensing data from the South Pole Telescope and Planck, obtaining the highest precision lensing ratio measurements to date. Relative to the concordance $\Lambda$CDM model, we find a best fit lensing ratio amplitude of $A = 1.1 \pm 0.1$. We use the ratio measurements to generate cosmological constraints, focusing on the curvature parameter. We demonstrate that photometrically selected galaxies can be used to measure lensing ratios, and argue that future lensing ratio measurements with data from a combination of LSST and Stage-4 CMB experiments can be used to place interesting cosmological constraints, even after considering the systematic uncertainties associated with photometric redshift and galaxy shear estimation.

==> Cosmological Constraints from Lensing Ratios/affil.tex <==
\section{Affiliations}
\textit{
$^{1}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{2}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{3}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{4}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{5}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08193 Barcelona, Spain\\
$^{6}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{7}$ Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{8}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL, 60637, USA\\
$^{9}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{10}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{11}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{12}$ Department of Astronomy/Steward Observatory, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{13}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{14}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{15}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
$^{16}$ Einstein Fellow\\
$^{17}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{18}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{19}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$^{20}$ Department of Physics and McGill Space Institute, McGill University, Montreal, Quebec H3A 2T8, Canada\\
$^{21}$ Canadian Institute for Advanced Research, CIFAR Program in Gravity and the Extreme Universe, Toronto, ON, M5G 1Z8, Canada\\
$^{22}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{23}$ Department of Physics, University of Illinois Urbana-Champaign, 1110 W. Green Street, Urbana, IL 61801, USA\\
$^{24}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{25}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{26}$ School of Physics, University of Melbourne, Parkville, VIC 3010, Australia\\
$^{27}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{28}$ Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK\\
$^{29}$ Cerro Tololo Inter-American Observatory, National Optical Astronomy Observatory, Casilla 603, La Serena, Chile\\
$^{30}$ Department of Physics and Electronics, Rhodes University, PO Box 94, Grahamstown, 6140, South Africa\\
$^{31}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{32}$ Department of Physics, University of California, Davis, CA, USA 95616\\
$^{33}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{34}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{35}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{36}$ High Energy Physics Division, Argonne National Laboratory, Argonne, IL, USA 60439\\
$^{37}$ Department of Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{38}$ Enrico Fermi Institute, University of Chicago, Chicago, IL 60637, USA\\
$^{39}$ National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{40}$ California Institute of Technology, Pasadena, CA, USA 91125\\
$^{41}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{42}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{43}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{44}$ Excellence Cluster Universe, Boltzmannstr.\ 2, 85748 Garching, Germany\\
$^{45}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{46}$ Center for Astrophysics and Space Astronomy, Department of Astrophysical and Planetary Sciences, University of Colorado, Boulder, CO, 80309\\
$^{47}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{48}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{49}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{50}$ Department of Physics, University of California, Berkeley, CA, USA 94720\\
$^{51}$ European Southern Observatory, Karl-Schwarzschild-Stra{\ss}e 2, 85748 Garching, Germany\\
$^{52}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{53}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{54}$ Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA, USA 94720\\
$^{55}$ Department of Physics, University of Colorado, Boulder, CO, 80309\\
$^{56}$ University of Chicago, Chicago, IL 60637, USA\\
$^{57}$ Harvard-Smithsonian Center for Astrophysics, Cambridge, MA 02138, USA\\
$^{58}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{59}$ Australian Astronomical Observatory, North Ryde, NSW 2113, Australia\\
$^{60}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{61}$ Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721\\
$^{62}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{63}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{64}$ Department of Physics, University of Chicago, Chicago, IL, USA 6063\\
$^{65}$ Dunlap Institute for Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada\\
$^{66}$ Department of Physics, University of Minnesota, Minneapolis, MN, USA 55455\\
$^{67}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{68}$ Physics Department, Center for Education and Research in Cosmology and Astrophysics, Case Western Reserve University,Cleveland, OH, USA 44106\\
$^{69}$ Liberal Arts Department, School of the Art Institute of Chicago, Chicago, IL, USA 60603\\
$^{70}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{71}$ Brandeis University, Physics Department, 415 South Street, Waltham MA 02453\\
$^{72}$ Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil\\
$^{73}$ Dept. of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305\\
$^{74}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{75}$ Department of Astronomy \& Astrophysics, University of Toronto, 50 St George St, Toronto, ON, M5S 3H4, Canada\\
$^{76}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$^{77}$ Berkeley Center for Cosmological Physics, Department of Physics, University of California, and Lawrence Berkeley National Labs, Berkeley, CA, USA 94720\\
}

==> Cosmological Constraints from Lensing Ratios/authorlist.tex <==
\author[Prat, Baxter et al.]{
\parbox{\textwidth}{
{\fontsize{11.3}{12} \selectfont 
J.~Prat$^{1}$\thanks{E-mail: jprat@ifae.es},
E.~Baxter$^{2}$\thanks{E-mail: ebax@sas.upenn.edu},
T.~Shin$^{2}$,
C.~S{\'a}nchez$^{2}$,
C.~Chang$^{3}$,
B.~Jain$^{2}$,
R.~Miquel$^{4,1}$,
A.~Alarcon$^{5,6}$,
D.~Bacon$^{7}$,
G.~M.~Bernstein$^{2}$,
R.~Cawthon$^{3}$,
T.~M.~Crawford$^{3,8}$,
C.~Davis$^{9}$,
J.~De~Vicente$^{10}$,
S.~Dodelson$^{11}$,
T.~F.~Eifler$^{12,13}$,
O.~Friedrich$^{14,15}$,
M.~Gatti$^{1}$,
D.~Gruen$^{16,9,17}$,
W.~G.~Hartley$^{18,19}$,
G.~P.~Holder$^{20,21,22,23}$,
B.~Hoyle$^{14,15}$,
M.~Jarvis$^{2}$,
E.~Krause$^{12}$,
N.~MacCrann$^{24,25}$,
B.~Mawdsley$^{7}$,
A.~Nicola$^{19}$,
Y.~Omori$^{9}$,
A.~Pujol$^{5,6}$,
M.~M.~Rau$^{11,15}$,
C.~L.~Reichardt$^{26}$,
S.~Samuroff$^{11}$,
E.~Sheldon$^{27}$,
M.~A.~Troxel$^{24,25}$,
P.~Vielzeuf$^{1}$,
J.~Zuntz$^{28}$,
T.~M.~C.~Abbott$^{29}$,
F.~B.~Abdalla$^{18,30}$,
J.~Annis$^{31}$,
S.~Avila$^{7}$,
K.~Aylor$^{32}$,
B.~A.~Benson$^{31,3,33}$,
E.~Bertin$^{34,35}$,
L.~E.~Bleem$^{36,3}$,
D.~Brooks$^{18}$,
D.~L.~Burke$^{9,17}$,
J.~E.~Carlstrom$^{3,37,36,33,38}$,
M.~Carrasco~Kind$^{22,39}$,
J.~Carretero$^{1}$,
C.~L.~Chang$^{36,3,33}$,
H-M.~Cho$^{17}$,
R.~Chown$^{20}$,
A.~T.~Crites$^{40}$,
C.~E.~Cunha$^{9}$,
L.~N.~da Costa$^{41,42}$,
S.~Desai$^{43}$,
H.~T.~Diehl$^{31}$,
J.~P.~Dietrich$^{44,45}$,
M.~A.~Dobbs$^{20,21}$,
P.~Doel$^{18}$,
W.~B.~Everett$^{46}$,
A.~E.~Evrard$^{47,48}$,
B.~Flaugher$^{31}$,
P.~Fosalba$^{5,6}$,
J.~Garc\'ia-Bellido$^{49}$,
E.~Gaztanaga$^{5,6}$,
E.~M.~George$^{50,51}$,
D.~W.~Gerdes$^{47,48}$,
T.~Giannantonio$^{52,53,15}$,
R.~A.~Gruendl$^{22,39}$,
J.~Gschwend$^{41,42}$,
G.~Gutierrez$^{31}$,
T.~de~Haan$^{50,54}$,
N.~W.~Halverson$^{46,55}$,
N.~L.~Harrington$^{50}$,
W.~L.~Holzapfel$^{50}$,
K.~Honscheid$^{24,25}$,
Z.~Hou$^{3,33}$,
J.~D.~Hrubes$^{56}$,
D.~J.~James$^{57}$,
T.~Jeltema$^{58}$,
L.~Knox$^{32}$,
R.~Kron$^{31,3}$,
K.~Kuehn$^{59}$,
N.~Kuropatkin$^{31}$,
O.~Lahav$^{18}$,
A.~T.~Lee$^{50,54}$,
E.~M.~Leitch$^{3,33}$,
M.~Lima$^{60,41}$,
D.~Luong-Van$^{56}$,
M.~A.~G.~Maia$^{41,42}$,
A.~Manzotti$^{3,33}$,
D.~P.~Marrone$^{61}$,
J.~L.~Marshall$^{62}$,
J.~J.~McMahon$^{48}$,
P.~Melchior$^{63}$,
F.~Menanteau$^{22,39}$,
S.~S.~Meyer$^{3,33,38,64}$,
C.~J.~Miller$^{47,48}$,
L.~M.~Mocanu$^{3,33}$,
J.~J.~Mohr$^{44,45,14}$,
T.~Natoli$^{3,37,65}$,
S.~Padin$^{3,33}$,
A.~A.~Plazas$^{13}$,
C.~Pryke$^{66}$,
A.~K.~Romer$^{67}$,
A.~Roodman$^{9,17}$,
J.~E.~Ruhl$^{68}$,
E.~S.~Rykoff$^{9,17}$,
E.~Sanchez$^{10}$,
J.~T.~Sayre$^{68,46}$,
V.~Scarpine$^{31}$,
K.~K.~Schaffer$^{3,38,69}$,
S.~Serrano$^{5,6}$,
I.~Sevilla-Noarbe$^{10}$,
E.~Shirokoff$^{50,3,33}$,
G.~Simard$^{20}$,
M.~Smith$^{70}$,
M.~Soares-Santos$^{71}$,
F.~Sobreira$^{72,41}$,
Z.~Staniszewski$^{68,13}$,
A.~A.~Stark$^{57}$,
K.~T.~Story$^{9,73}$,
E.~Suchyta$^{74}$,
M.~E.~C.~Swanson$^{39}$,
G.~Tarle$^{48}$,
D.~Thomas$^{7}$,
K.~Vanderlinde$^{65,75}$,
J.~D.~Vieira$^{22,23}$,
V.~Vikram$^{76}$,
A.~R.~Walker$^{29}$,
J.~Weller$^{44,14,15}$,
R.~Williamson$^{3,33}$,
O.~Zahn$^{77}$
\begin{center} (The DES and SPT Collaborations) \end{center}
}}
\vspace{0.4cm}
\\
\parbox{\textwidth}{Author affiliations are listed at the end of the paper}}

==> Cosmological Constraints from Lensing Ratios/notations.tex <==
% cosmological parameters
\newcommand{\om}{\Omega_\mr m}
\newcommand{\omb}{\Omega_\mr b}
\newcommand{\ns}{n_s}
\newcommand{\w}{w_0}
\newcommand{\wa}{w_a}

% units
\newcommand{\uk}{\mu K}
\newcommand{\mjy}{{\rm mJy}}
\newcommand{\emm}{ \textit{m}\ }
\newcommand{\sqdeg}{{\rm deg}^{2}}

% cls
\newcommand{\clpp}{\hat C_{L}^{\phi\phi}}
\newcommand{\clxx}{\hat C_{L}^{\psi\psi}}
\newcommand{\clpg}{\hat C_{L}^{\phi G}}

% real space correlation functions
\def\galk{w^{\delta_g \kappa_{\rm CMB}}(\theta) }
\def\galik{w^{\delta_g^i \kappa_{\rm CMB}}(\theta) }
\def\sheark{w^{\gamma \kappa_{\rm CMB}}(\theta)}
\def\sheartk{w^{\gamma_T \kappa_{\rm CMB}}(\theta)}
\def\sheartik{w^{\gamma^i_T \kappa_{\rm CMB}}(\theta)}
\def\kk{w^{\kappa_{\rm CMB}\kappa_{\rm CMB}}(\theta)}
\def\galkobs{w^{\delta_g \kappa_{\rm obs}}(\theta)}
\def\galksim{w^{\delta_g \kappa_{\rm sim}}(\theta)}
\def\galksys{w^{\delta_g \kappa_{\rm sys}}(\theta)}
\def\galktsz{w^{\delta_g \kappa_{\rm tSZ}}(\theta)}
\def\shearkobs{w^{\gamma \kappa_{\rm obs}}(\theta)}
\def\sheartkobs{w^{\gamma_T \kappa_{\rm obs}}(\theta)}
\def\sheartksim{w^{\gamma_T \kappa_{\rm sim}}(\theta)}
\def\sheartktsz{w^{\gamma_T \kappa_{\rm tSZ}}(\theta)}
\def\shearksys{w^{\gamma \kappa_{\rm sys}}(\theta)}
\def\sheartksys{w^{\gamma_T \kappa_{\rm sys}}(\theta)}

% 3x2pt correlations
\def\galgal{w^{\delta_g \delta_g}(\theta)}
\def\galshear{w^{\delta_g \gamma}(\theta)}
\def\galsheart{w^{\delta_g \gamma_T}(\theta)}
\def\shearshear{w^{\gamma \gamma}(\theta)}
\def\wtheta{w^{\delta_g \delta_g}(\theta)}
\def\gglensing{w^{\delta_g \gamma}(\theta)}

%harmonic space correlation functions
\def\galkell{C^{\delta_g \kappa_{\rm CMB}} (\ell)}
\def\galikell{C^{\delta_g^i \kappa_{\rm CMB}} (\ell)}
\def\galktszell{C^{\delta_g \kappa_{\rm tSZ}} (\ell)}
\def\kappaskell{C^{\kappa_s \kappa_{\rm CMB}}(\ell)}
\def\kappasikell{C^{\kappa_s \kappa_{\rm CMB}}(\ell)}
\def\kappasktszell{C^{\kappa_s \kappa_{\rm tSZ}}(\ell)}


%joint correlation functions
\def\3x2pt{3$\times$2pt}
\def\5x2pt{5$\times$2pt}
\def\6x2pt{6$\times$2pt}

% experiments
\newcommand{\sptp}{{\rm SPT}+\textit{Planck}}
\newcommand{\planck}{\textit{Planck}}
\newcommand{\wmap}{\textit{WMAP}}
\newcommand{\des}{\textsc{DES}}

% measurements
\newcommand{\kcmb}{\kappa_{\rm CMB}}
\newcommand{\ktsz}{\kappa_{\rm tSZ}}
\newcommand{\kcib}{\kappa_{\rm CIB}}
\newcommand{\kgal}{\kappa_{\rm g}}

\newcommand{\ktszcib}{\kappa_{\rm tSZ/CIB}}

\newcommand{\gammat}{\gamma_{\rm t}}
\newcommand{\gammax}{\gamma_{\times}}
\newcommand{\kE}{\kappa_{\rm E}}
\newcommand{\kB}{\kappa_{\rm B}}
\newcommand{\delg}{\delta_{\rm g}}
\newcommand{\fk}{f_{K}}



%codes
\newcommand{\imshape}{\textsc{Im3shape}}
\newcommand{\ngmix}{\textsc{ngmix}}
\newcommand{\cosmolike}{\textsc{CosmoLike}}
\newcommand{\cosmosis}{\textsc{CosmoSIS}}
\newcommand{\cosmomc}{\textsc{CosmoMC}}
\newcommand{\polspice}{\textsc{PolSpice}}
\newcommand{\treecorr}{\textsc{TreeCorr}}
\newcommand{\quicklens}{\textsc{Quicklens}}
\newcommand{\metacal}{\textsc{Metacalibration}}
\newcommand{\flask}{\textsc{Flask}}
\newcommand{\gnilc}{\textsc{GNILC}}
\newcommand{\healpix}{\textsc{HEALPix}}
\newcommand{\redmagic}{\textsc{redMaGiC}}
\newcommand{\redmapper}{\textsc{redMaPPer}}

